BenchScope: How Many Independent Signals Does Your Benchmark Provide?

AI evaluation suites often report many scores without checking whether those scores carry independent information. We introduce Effective Dimensionality (ED), the participation ratio of a centered benchmark-score spectrum, as a fast, population-conditional upper-bound diagnostic of measurement breadth. Applied at per-instance granularity to 22 benchmarks across 8 domains and more than 8,400 model evaluations, ED reveals substantial redundancy: the six-score Open LLM Leaderboard behaves like roughly two effective measurement axes (ED = 1.7), BBH and MMLU-Pro are near-interchangeable (rho = 0.96, stable across seven subpopulations), and measurement breadth varies more than 20x across current benchmarks. We show that relative ED rankings are stable under matched-dimension controls and that ED can flag redundant suite components, monitor performance-conditional compression, and guide benchmark maintenance. Because binary spectra overestimate absolute latent dimensionality, we interpret ED as a screening statistic rather than a literal factor count and complement it with null, reliability, and saturation analyses. We provide a 22-benchmark reference atlas and a four-step diagnostic workflow that benchmark maintainers can run with a score matrix and a few lines of code.

==> sections/theory.tex <==
% !TEX root = ../main.tex
% NOTE: This file is transitional. Its contents will be redistributed:
%   - ED-Greedy → criteria.tex (diagnostic workflow section)
%   - Composite ceiling → redundancy_tradeoffs.tex (conditional correlations subsection)
% After redistribution, this file will be removed from main.tex.

\section{Applications and Supporting Theory}
\label{sec:theory}

%------------------------------------------------------------------
\subsection{ED-Greedy: Principled Task Selection}
\label{sec:ed-greedy}
%------------------------------------------------------------------

The spectral framework suggests a constructive application: instead of merely diagnosing redundancy post hoc, we can optimize benchmark composition to maximize ED.
We formulate this as a combinatorial optimization problem: given a candidate pool of $T$ tasks and a budget of $k \leq T$, select the subset $S^* \subseteq [T]$ with $|S^*| = k$ that maximizes $\text{ED}(M_S)$, where $M_S$ is the submatrix of $M$ restricted to the rows in $S$.
This objective directly optimizes for measurement diversity---the number of independent capability axes the selected tasks span.

We propose \textsc{ED-Greedy} (Algorithm~\ref{alg:ed-greedy}): starting from an empty set, iteratively add the task that produces the largest marginal increase in ED.
Each iteration requires computing ED for at most $T$ candidate additions, each involving an SVD of an $(|S|{+}1) \times N$ matrix, giving total complexity $O(k \cdot T \cdot N^2)$---fast enough for practical use even with thousands of candidate tasks.
The greedy strategy is a natural choice because ED, like other participation-ratio-based objectives, favors spreading variance across components; adding a task that is redundant with the current set contributes variance along an already-dominant axis, producing little marginal gain.

\begin{algorithm}[htbp]
\caption{\textsc{ED-Greedy}: Task Selection for Maximum Effective Dimensionality}
\label{alg:ed-greedy}
\begin{algorithmic}[1]
\REQUIRE Pass/fail matrix $M \in \{0,1\}^{T \times N}$, budget $k$
\ENSURE Selected task set $S^*$ with $|S^*| = k$
\STATE $S \leftarrow \emptyset$
\FOR{$i = 1$ to $k$}
  \STATE $t^* \leftarrow \arg\max_{t \in [T] \setminus S}\; \text{ED}(M_{S \cup \{t\}})$
  \STATE $S \leftarrow S \cup \{t^*\}$
\ENDFOR
\RETURN $S$
\end{algorithmic}
\end{algorithm}

If ED were submodular as a set function, the greedy algorithm would achieve a $(1 - 1/e) \approx 0.63$ approximation to the optimal subset~\citep{nemhauser1978}.
Empirically, ED is approximately submodular: on BigCodeBench, the median submodularity ratio across random subset pairs is $\gamma = 0.64$, but edge cases exist where the ratio drops to zero, precluding a formal worst-case guarantee.
In practice, ED-Greedy vastly outperforms random selection in maximizing ED: at $k = 50$ tasks, ED-Greedy achieves $\text{ED} = 37.8$ versus $4.2$ for a random subset of equal size.

An important distinction: ED-Greedy maximizes measurement diversity (the number of independent axes), not rank preservation (how well a subset reproduces the full ranking).
We compared six task-selection methods on BigCodeBench (300 tasks, 153 models): ED-Greedy, random, max-variance, IRT-inspired (highest discrimination), $k$-medoids clustering, and a two-stage method (ED-Greedy selects $2k$ tasks, then IRT picks the $k$ most discriminating).
At $k = 10$, IRT-inspired achieves the highest $\tau$ ($0.77$) while ED-Greedy achieves the highest ED ($8.6$, $\tau = 0.53$).
At $k = 50$, ED-Greedy achieves both high ED ($33.7$) and competitive $\tau$ ($0.85$), comparable to IRT ($\tau = 0.84$); the two-stage method is a slight compromise ($\text{ED} = 31.0$, $\tau = 0.83$).
At $k \geq 100$, all methods converge in $\tau$ (${\sim}0.87$), but ED-Greedy retains a large ED advantage ($38.1$ vs.\ $4.1$ for random).
The IRT-inspired baseline is conceptually similar to the tinyBenchmarks approach of \citet{polo2024tinybenchmarks}, which also selects high-discrimination items for rank preservation; ED-Greedy optimizes a complementary objective (measurement diversity) that tinyBenchmarks does not target.

\paragraph{ED tracks compression difficulty.}
We measured how many tasks a benchmark needs to achieve $\tau \geq 0.95$ with the full-task ranking, across eight benchmarks with $T \geq 100$ per-instance items.\footnote{MMLU-Pro and BBH use expanded model matrices (118 and 113 models, respectively) from the Open LLM Leaderboard per-question results, yielding higher ED than the smaller matrices in Table~\ref{tab:reference}.}
Higher-ED benchmarks generally need more tasks (Spearman $\rho = 0.64$, $n = 8$):

\begin{center}
\small
\begin{tabular}{lrrr}
\toprule
\textbf{Benchmark} & \textbf{ED} & \textbf{Tasks needed} & \textbf{Compression} \\
\midrule
BFCL            & 1.5  & 8\%  & $12.7\times$ \\
LiveCodeBench   & 6.2  & 17\% & $5.9\times$ \\
AlpacaEval~2.0  & 7.3  & 41\% & $2.4\times$ \\
SWE-bench       & 7.9  & 43\% & $2.3\times$ \\
IFEval          & 12.6 & 46\% & $2.2\times$ \\
MMLU-Pro        & 20.8 & 19\% & $5.3\times$ \\
BBH             & 26.6 & 26\% & $3.8\times$ \\
BigCodeBench    & 28.9 & 56\% & $1.8\times$ \\
\bottomrule
\end{tabular}
\end{center}
The general direction is clear---higher-ED benchmarks require more tasks to preserve ranking structure---but two exceptions reveal that ED alone is not a perfect predictor of compression cost.
MMLU-Pro and BBH have high ED ($20$--$27$) yet compress relatively easily ($3.8$--$5.3\times$); their large task pools ($T > 5{,}000$) include substantial internal redundancy that random sampling efficiently averages out.
The practical lesson: ED flags which benchmarks cannot be aggressively compressed (high ED + moderate $T$, e.g., BigCodeBench), but for benchmarks with very large $T$, internal item redundancy matters as much as spectral diversity.

\paragraph{Prospective generalization.}
ED-Greedy is a diagnostic tool for understanding benchmark structure, not a turnkey benchmark-design method.
To test prospective validity, we split each benchmark's models by performance into a design cohort (bottom 60\%) and a future cohort (top 40\%), selected tasks on the design set, and evaluated $\tau$ on the future set.
On SWE-bench, ED-Greedy beats random on the future cohort at $k = 10, 50, 100$ (e.g., $\tau = 0.81$ vs.\ $0.77$ at $k = 100$), with a mean generalization gap of only $-0.01$---essentially no overfitting.
In contrast, the high-variance baseline catastrophically overfits: its train $\tau$ exceeds $0.88$ but its test $\tau$ drops to $0.37$--$0.58$.
On low-ED benchmarks (BFCL, $\text{ED} = 1.5$), random selection is already near-optimal because the benchmark has only one effective dimension to capture.

%------------------------------------------------------------------
\subsection{Why Low ED Makes Composite Scores Lossy}
\label{sec:composite-theory}
%------------------------------------------------------------------

When two benchmarks are negatively correlated within a subpopulation, the composite ranking is mathematically unable to faithfully represent both---not merely empirically unstable.

\begin{theorem}[Composite correlation ceiling]
\label{thm:composite}
Let $s_1, s_2$ be standardized benchmark scores with Pearson correlation $\rho$.
For any composite $c = w_1 s_1 + w_2 s_2$ with $w_1, w_2 > 0$:
\begin{equation}
  \max_{w_1, w_2 > 0}\;\min\!\big(\mathrm{corr}(c, s_1),\;\mathrm{corr}(c, s_2)\big) \;=\; \sqrt{\frac{1 + \rho}{2}}\,.
  \label{eq:composite-ceiling}
\end{equation}
The maximum is attained at equal weights $w_1 = w_2$.
\end{theorem}

\begin{proof}
Set $w_1 = 1$ without loss of generality and let $t = w_2 > 0$.
Then $r_1(t) = (1 + t\rho)/\sqrt{1 + t^2 + 2t\rho}$ and $r_2(t) = (t + \rho)/\sqrt{1 + t^2 + 2t\rho}$.
The symmetry $r_1(t) = r_2(1/t)$ implies that $r_1$ and $r_2$ cross at $t = 1$.
For $t < 1$: $r_1(t) - r_2(t) = (1 - t)(1 - \rho)/\sqrt{1 + t^2 + 2t\rho} > 0$ (since $\rho < 1$), so $r_1 > r_2$.
For $t > 1$: the sign reverses, so $r_2 > r_1$.
Therefore $\min(r_1, r_2)$ equals $r_2$ for $t < 1$ and $r_1$ for $t > 1$; it is maximized at the crossing point $t = 1$, where both equal $(1+\rho)/\sqrt{2(1+\rho)} = \sqrt{(1+\rho)/2}$.
\end{proof}

\noindent
The theorem assumes positive weights ($w_1, w_2 > 0$), standard for leaderboard composites.
The result holds for Pearson correlation; because the empirical correlations in Table~\ref{tab:tradeoffs} are Spearman rank correlations, the ceiling values are approximate (Pearson--Spearman discrepancy is typically $< 0.03$ in our data).

\paragraph{Information density.}
Define the information density of a $k$-benchmark suite as $\text{ID} = \text{ED}/k$, measuring the ratio of independent signals to reported scores.
For the Open LLM Leaderboard v2, $\text{ID} = 1.7/6 = 0.28$: only 28\% of the reported scores carry independent information.

